Counter-Empirical Attacking based on Adversarial Reinforcement Learning for Time-Relevant Scoring System

Scoring systems are commonly seen for platforms in the era of big data. From credit scoring systems in financial services to membership scores in E-commerce shopping platforms, platform managers use such systems to guide users towards the encouraged activity pattern, and manage resources more effectively and more efficiently thereby. To establish such scoring systems, several "empirical criteria" are firstly determined, followed by dedicated top-down design for each factor of the score, which usually requires enormous effort to adjust and tune the scoring function in the new application scenario. What's worse, many fresh projects usually have no ground-truth or any experience to evaluate a reasonable scoring system, making the designing even harder. To reduce the effort of manual adjustment of the scoring function in every new scoring system, we innovatively study the scoring system from the preset empirical criteria without any ground truth, and propose a novel framework to improve the system from scratch. In this paper, we propose a "counter-empirical attacking" mechanism that can generate "attacking" behavior traces and try to break the empirical rules of the scoring system. Then an adversarial "enhancer" is applied to evaluate the scoring system and find the improvement strategy. By training the adversarial learning problem, a proper scoring function can be learned to be robust to the attacking activity traces that are trying to violate the empirical criteria. Extensive experiments have been conducted on two scoring systems including a shared computing resource platform and a financial credit system. The experimental results have validated the effectiveness of our proposed framework.

==> problem_formulation.tex <==
% \section{Preliminaries}
\section{Problem Formulation}\label{sec:pre}
% \subsection{Scenario Setting}
We formulate the research problem in this paper as follows.
In a platform where each user $i$ can take an activity $a_t$ from action space $\mathcal{A}$ in each time step $t$, a typical scoring system scores each user at each time step. 
% Thus the output score of the user can be represented as:
We can represent the output score of the user as:
\begin{equation}
    \{S_i^t\}_{i=1,\ldots,N}
\end{equation}
where $N$ is the number of users in the system, and $S_i^t$ denotes the score of user $i$ at time step $t$. 
The scores can be obtained according to users' basic information and past activities on the platform, and the specific form of the scoring function mapping the user features to the final scores can be very flexible. Generally, the function form is the sum of a set of base values calculated with static user features such as gender and age, and a set of factors related to users' activity records on the platform. As the factors developed from static user information usually remain unchanged upon new activities, we only target on the factors related to users' activity records, and call the score for these factors the scoring function. 
Although our methodology does not require any specific form of the scoring function, here we show a common form of scoring functions that is prone to be attacked by deliberately designed activities to violate preset empirical criteria.  

\subsubsection*{Scoring Function}
% because we only evaluate the robustness of the scoring function by along the activity traces for each individual in this work. 
A typical scoring function for user $i$ at time step $t$ is the sum of several time-relevant factor modules:
\begin{equation}
\label{eqn:score_form}
    S_i^t = \sum_{k=1}^K w_k \cdot m_{k}(t, \phi_k, \mathcal{H}^t_i)
\end{equation}
where $w_k$ is the weight for the $k^{\textrm{th}}$ factor module and $m_{k}(t, \phi_k, \mathcal{H}^t_i)$ is the module score for the $k^{\textrm{th}}$ time-relevant factor module, with $\phi_k$ being the parameters inside the module function and $\mathcal{H}^t_i = \{a_t, a_{t-1}, \ldots\}$ is the historical activities of user $i$ for calculating each module score. \red{In Appendix \ref{sec:app}, we present two examples of scoring functions in different applications. }

\subsubsection*{Empirical Criteria}
In the designing stage of a scoring function in the form of (\ref{eqn:score_form}), there is a set of ``empirical criteria'' in the following form: 
\begin{equation}
\label{eqn:empirical_cri}
    S_i^t < S_i^{t+1} \textrm{ if } a_i^t \prec a_{i}^{t+1} 
\end{equation}
where $a_i^t$ and $a_i^{t+1}$ represent the activities for user $i$  at time $t$ and $t+1$ respectively, and $\prec \subset \mathcal{A}^2$  represents a partial order for a pair of activities. One example of an activity is repaying all the loan in the financial credit scoring application. Note that here the two compared activities do not need to be of the same type, as long as the deduced empirical criteria is reasonable in the application. Besides, we don't require the set of empirical criteria cover all types of activities.
Since these empirical criteria are applied on two activities of a user, they can effectively encode the intuitive expectations to the scoring systems.
% are usually proposed by the designers of such scoring systems and have intuitive explanations. 
If (\ref{eqn:empirical_cri}) fails to be satisfied, we call there is a violation of this empirical criterion. 


\subsubsection*{Objective} Our goal in this work is to learn the parameters  $\Phi = (\bm w, \bm \phi)$, $\bm w = (w_1,\ldots,w_K)$, $\bm \phi = (\phi_1,\ldots, \phi_K)$  for the scoring function so as to minimize the expected frequency of counter cases weighted over their severity against the preset empirical criteria. Due to the complexity of the function brought by the time-relevant factors (usually representing the decaying effect of past activities on current scores), the preset empirical criteria are prone to violate by some deliberately designed activity traces. To learn a more robust scoring function against these activity traces, we adopt the adversarial learning framework in our proposed method, which will be explained in detail in the following section.


